Specialized minimal PDFs for optimized LHC calculations

We present a methodology for the construction of parton distribution functions (PDFs) designed to provide an accurate representation of PDF uncertainties for specific processes or classes of processes with a minimal number of PDF error sets: specialized minimal PDF sets, or SM-PDFs. We construct these SM-PDFs in such a way that sets corresponding to different input processes can be combined without losing information, specifically on their correlations, and that they are robust upon smooth variations of the kinematic cuts. The proposed strategy never discards information, so that the SM-PDF sets can be enlarged by the addition of new processes, until the prior PDF set is eventually recovered for a large enough set of processes. We illustrate the method by producing SM-PDFs tailored to Higgs, top quark pair, and electroweak gauge boson physics, and determine that, when the PDF4LHC15 combined set is used as the prior, around 11, 4 and 11 Hessian eigenvectors respectively are enough to fully describe the corresponding processes.

==> referee.tex <==
We thank the referee for his insightful comments.


The discussion of the perturbative order was indeed quite unclear. We
have added a new paragraph which explicitly addresses it: next-to-last
paragraph of Sect 2.3, starting with ``The SM_PDF construction''. We
have further added a brief comment in this respect in sect 3.1: last
two sentences of the first paragraph of sect 3.1, starting with ``As
already mentioned''.

The suggestion of the referee to make an explicit comparison of the
``ladder'' SM-PDF set to the PDF4LHC15 sets is so good that we have
already made this comparison! In fact, we have submitted it to the Les
Houches proceedings a few weeks ago, and it will appear on the arXiv
as soon as the proceedings are released. We have added an explicit
reference to this, as the last sentence of Sect.3.3 (starting with 
``In fact we have explicitly checked...'')
We attach a copy of our Les Houches contribution so that the referee
can check explicitly the statement we make here,

Finally, we have corrected all the typos found by the referee and we
would like to thank him for carefully checking our manuscript.


